Crowdsourcing the Perception of Machine Teaching

Teachable interfaces can empower end-users to attune machine learning systems to their idiosyncratic characteristics and environment by explicitly providing pertinent training examples. While facilitating control, their effectiveness can be hindered by the lack of expertise or misconceptions. We investigate how users may conceptualize, experience, and reflect on their engagement in machine teaching by deploying a mobile teachable testbed in Amazon Mechanical Turk. Using a performance-based payment scheme, Mechanical Turkers (N = 100) are called to train, test, and re-train a robust recognition model in real-time with a few snapshots taken in their environment. We find that participants incorporate diversity in their examples drawing from parallels to how humans recognize objects independent of size, viewpoint, location, and illumination. Many of their misconceptions relate to consistency and model capabilities for reasoning. With limited variation and edge cases in testing, the majority of them do not change strategies on a second training attempt.

==> alternative_text.tex <==
[fig:category_samples]
This figure shows six photos and a symbol for each category. The six photos are from two participants who had 3 photos of different objects for each. Within a category, six photos are shown at the top with participants indices below the photos and a symbol below the participants indices. The categories are aligned from left to right in order of bottle, cereal, drink, snack, and spice. The photos of bottles are from P19 and P25. The photos of cereals are from P3 and P18. The photos of drinks are from P6 and P33. The photos of snacks are from P8 and P46. The photos of spices are from P1 and P2.

[fig:screenshot]
This figure includes eight images that are screenshots of web interfaces for different steps of the user study. The images are aligned horizontally from left to right. The first and second image shows the interface of background questions with text boxes and radio buttons. The third image shows the interface for selecting the category of objects. It shows a drop down list at the top and examples photos of the objects below. The fourth image shows three text boxes for participants to enter the name of the object instances. The fifth image shows a camera interface with a name of the object that participant was supposed to capture in the photo. The sixth image is showing a incorrect prediction result in a black box and white text on top of the camera interface. The seventh image is camera interface for training with thumbnail of previous image at the bottom left. The eighth image is the same interface as sixth image, but with correct prediction result.

[MachineTeachingConcept]
This figure shows the feature of the machine learning task in a table form. A row consists of the name of category and list of features aligned horizontally. The features that belongs to the teachable object recognizer are highlighted. The features are described as follows.
Human vs. machine: T=machine/S=machine, T=machine/S=student, T=human/S=machine (highlighted), T=human/S=human
Teaching signal: synthetic/constructive teaching, hybrid teaching, pool-based teaching (highlighted)
Model-based vs. model-free: model-based teaching, graybox teaching, model-free teaching (highlighted)
Angelic vs. adversarial: angelic teaching (highlighted), adversarial teaching
Batch vs. sequential: batch learning (highlighted), sequential learning
Student awareness: the student anticipates teaching, the student does not anticipate teaching (highlighted)
One vs. many: one student (highlighted), many student
Theoretical vs. empirical: theoretical teaching, hybrid, empirical teaching (highlighted)


[concept_diagram]
This figure shows a block diagram with blocks as components that affect the performance of TOR and links as relations of the components. The blocks include experience (first and second use of teachable interface), object (5 categories of object), performance (accuracy of recognizing objects), behavior (patterns of taking photos). The links are from experience to performance, from experience to behavior, from object to performance, from object to behavior, and from behavior to performance.

[fig:chart_background]
This figure is a bar chart describing participants background.

Statement: Use a mobile device.
Never: 1%
Once a month: 0%
Several times a month: 0%
Once a week: 0%
Several times a week: 0%
Once a day: 1%
Several times a day: 98%

Statement: Take pictures using a mobile phone.
Never: 0%
Once a month: 0%
Several times a month: 9%
Once a week: 4%
Several times a week: 42%
Once a day: 19%
Several times a day: 26%

Statement: Use apps that can recognize type of objects, food, or plants through Never: 62%
Once a month: 13%
Several times a month: 10%
Once a week: 2%
Several times a week: 9%
Once a day: 2%
Several times a day: 2%

How would you classify your level of familiarity with machine learning?
Not familiar at all: 6%
Slightly familiar: 45%
Somewhat familiar: 48%
Extremely familiar: 1%



[chart_variation_inconistency]
This figure shows two bar charts. The bar chart on the left side shows the number of participants who included variations. The bar chart on the right side shows the number of participants with inconsistency of variation.
Number of participants with variation
TS0
VSizeDist: 49
VLoCBg: 20
VViewSide:11 
VViewAngle: 24
VViewPos: 6
VIllumExp: 4
VIllumSrc: 5
VNone: 76

TS1
VSizeDist: 57
VLoCBg: 21
VViewSide: 29
VViewAngle: 32
VViewPos: 17
VIllumExp: 0
VIllumSrc: 6
VNone: 56

TS2
VSizeDist: 48
VLoCBg: 16
VViewSide: 22
VViewAngle: 23
VViewPos: 23
VIllumExp: 3
VIllumSrc: 3
VNone: 63

TR1
VSizeDist: 65
VLoCBg: 39
VViewSide: 36 
VViewAngle: 53 
VViewPos: 39
VIllumExp: 4
VIllumSrc: 16
VNone: 41

TR2
VSizeDist: 59
VLoCBg: 28
VViewSide: 36
VViewAngle: 54
VViewPos: 39
VIllumExp: 8
VIllumSrc: 16
VNone: 41

Number of participants with inconsistency
TS0
ISize: 39
ILoc: 13
IView: 18
IIllum: 1

TS1
ISize: 39
ILoc: 10
IView: 24
IIllum: 1

TS2
ISize: 27
ILoc: 9
IView: 25
IIllum: 0

TR1
ISize: 23
ILoc: 10
IView: 31
IIllum: 5

TR2
ISize: 15
ILoc: 5
IView: 26
IIllum: 7



[fig:chart_presence]
This figure on the left shows a bar chart showing the average percentage of photos with the count features.

TS0
CCrop: 7.93%
CReshape: 0%
CContents: 0.2%
CNoBg: 7.3%
CPlainBg: 25.0%
CClutBg: 24.5%
CTextBg: 43.1%
CHands: 9.2%
CLogo: 94.1%
CFlash: 0.2%

TS1
CCrop: 10.5%
CReshape: 0.0%
CContents: 0.0%
CNoBg: 4.9%
CPlainBg: 15.1%
CClutBg: 36.3%
CTextBg: 43.6%
CHands: 10.7%
CLogo: 87.3%
CFlash: 0.0%

TS2
CCrop: 2.36
CReshape: 0
CContents: 0
CNoBg: 0.98
CPlainBg: 2.65
CClutBg: 4.17
CTextBg: 7.2
CHands: 0.92
CLogo: 13.37
CFlash: 0.05

TR1
CCrop: 9.04
CReshape: 1.19
CContents: 0.67
CNoBg: 3.83
CPlainBg: 16.88
CClutBg: 29.87
CTextBg: 39.4
CHands: 7.37
CLogo: 76.42
CFlash: 0.07

TR2
CCrop: 9.49
CReshape: 0.78
CContents: 0.87
CNoBg: 5.65
CPlainBg: 18.93
CClutBg: 27.93
CTextBg: 37.47
CHands: 9.23
CLogo: 75.85
CFlash: 0

This figure on the right shows a bar chart showing the average number of photos with the quality issues of count features.

TS0
QSmall: 0.01
QDim: 0.29
QBlurry: 0.51
QIrrelevant: 0.01

TS1
QSmall: 0.12
QDim: 0.45
QBlurry: 0.97
QIrrelevant: 0

TS2
QSmall: 0.1
QDim: 0.22
QBlurry: 0.77
QIrrelevant: 0.02

TR1
QSmall: 1.7
QDim: 1.94
QBlurry: 2.43
QIrrelevant: 0

TR2
QSmall: 0.78
QDim: 2.26
QBlurry: 3.24
QIrrelevant: 0.1

[samples_variation]
This figure has 7 rows of photos. Each row has 8 photos with a variation feature. The first row shows photos with VSizeDist feature. The second low shows photos with VLocBg feature. The third row shows photos with VViewSide feature. The fourth row shows VViewAngle feature. The fifth row shows photos with VViewPos feature. The sixth row shows VIllumExp feature. The seventh row shows the photos with VIllumSrc feature.

[samples_presence]
This figure shows 8 photos for each count feature except CFlash (5 photos). The photos with the same count feature is grouped together. There are 5 rows of photos. Two groups are positioned on the left and right in a row. From the top to bottom and left to right, the photos has CCrop, CClutBg, CReshape, CTextBg, CContents, CHands, CNoBg, CLogo, CPlainBg, and CFlash features.

[fig:relative_importance]
This figure shows a bar chart wich confidence interval for each bar.

[TR*TS]CCrop: 18.16% [3.49, 33.13]
[TR]VIllumExp: 16.09% [4.15, 25.21]
[TS]CCrop: 13.84% [4.37, 22.90]
[TS]VViewSide: 12.05% [2.60, 27.19]
[TS]VViewPos: 7.65% [0.46, 29.37]
[TR]CPlainBg: 7.42% [0.54, 28.70]
[TR]VIllumSrc: 6.01% [0.46, 22.12]
[TS]QBlurry: 5.01% [0.40, 20.10]
[TR]CCrop: 4.59% [2.34, 12.56]
[TS]VSizeDist: 4.04% [0.57, 20.29]
[TS]CClutBg: 3.35% [0.55, 10.02]
[TR]CTextBg: 1.80% [0.38, 12.14]

[category_shape]
This figure shows a bar chart showing the number of objects with 6 different shapes in 5 categories.

Bottle shape
Bottle: 43
Cereal: 0
Drink: 19
Snack: 0
Spice: 5

Box shape
Bottle: 0
Cereal: 44
Drink: 5
Snack: 5
Spice: 19

Cylinder shape
Bottle: 5
Cereal: 0
Drink: 28
Snack: 7
Spice: 96

Rectangle shape
Bottle: 0
Cereal: 0
Drink: 1
Snack:4
Spice: 3

SnackBag shape
Bottle: 0
Cereal: 1
Drink: 1
Snack: 13
Spice: 0

Sphere shape
Bottle: 0
Cereal: 0
Drink: 0
Snack: 1
Spice: 0



[category_fscore]
This figure shows a box plot showing the f-score of TORs trained with different categories of objects.

Average F-score
Bottle: 0.81 (min: 0.43, max: 1.0, std: 0.22, median: 0.97)
Cereal: 0.81 (min: 0.17, max: 1.0, std: 0.25, median: 0.93)
Drink: 0.87 (min: 0.17, max: 1.0, std: 0.22, median: 0.93)
Snack: 0.95 (min: 0.68, max: 1.0, std: 0.10, median: 1.0)
Spice: 0.59 (min: 0.11, max: 1.0, std: 0.28, median: 0.56)




